Non-Orthogonal Multiple-Access Strategies for Direct-to-Satellite IoT Networks

Direct-to-Satellite IoT (DtS-IoT) has the potential to support multiple verticals, including agriculture, industry, smart cities, and environmental disaster prevention. This work introduces two novel DtS-IoT schemes using power domain NonOrthogonal Multiple Access (NOMA) in the uplink with either fixed (FTP) or controlled (CTP) transmit power. We consider that the IoT devices use LoRa technology to transmit data packets to the satellite in orbit, equipped with a Successive Interference Cancellation (SIC)-enabled gateway. We also assume the IoT devices are empowered with a predictor of the satellite orbit. Using real geographic location and trajectory data, we evaluate the performance of the average number of successfully decoded transmissions, goodput (bytes/lap), and energy consumption (bytes/Joule) as a function of the number of network devices. Numerical results show the trade-off between goodput and energy efficiency for both proposed schemes. Comparing FTP and CTP with regular ALOHA for 100 (600) devices, we find goodput improvements of 65% (29%) and 52% (101%), respectively. Notably, CTP effectively leverages transmission opportunities as the network size increases, outperforming the other strategies. Moreover, CTP shows the best performance in energy efficiency compared to FTP and ALOHA.

==> Arquivos_Jan24/backup_main <==
%ESSE É UM BACKUP \documentclass[journal,10pt]{IEEEtran}


\usepackage{blindtext, graphicx}
\usepackage[english]{babel}
\usepackage[utf8]{inputenc}
\usepackage[T1]{fontenc}
\usepackage{multirow}
\usepackage[table]{xcolor}
\usepackage{graphics}

\usepackage{amsmath}
\hyphenation{op-tical net-works semi-conduc-tor}
\usepackage{enumerate}
\usepackage{xcolor}
\usepackage{amsfonts}
\usepackage{mathtools}
\usepackage{amssymb}
\usepackage{mathrsfs}
\usepackage{epstopdf}
\usepackage{graphicx}
\usepackage{cite}
\usepackage{soulutf8}
\usepackage{ragged2e}

\usepackage{graphicx}
\usepackage{subfig}

\usepackage{tabularray}

\usepackage{tablefootnote}
\usepackage[flushleft]{threeparttable}
\usepackage{pifont}% http://ctan.org/pkg/pifont
\usepackage{tikz}

\usepackage{mathtools, cuted}
\usepackage{lipsum, color}

\newcommand{\tikzxmark}{%
\tikz[scale=0.23] {
    \draw[line width=0.7,line cap=round] (0,0) to [bend left=6] (1,1);
    \draw[line width=0.7,line cap=round] (0.2,0.95) to [bend right=3] (0.8,0.05);
}}
\newcommand{\tikzcmark}{%
\tikz[scale=0.23] {
    \draw[line width=0.7,line cap=round] (0.25,0) to [bend left=10] (1,1);
    \draw[line width=0.8,line cap=round] (0,0.35) to [bend right=1] (0.23,0);
}}

%\usepackage{subcaption}

%\theoremstyle{definition}
\newtheorem{definition}{\textbf{Definition}}[section]

\newcommand\rds[1]{\textcolor{orange}{(#1)}}
\newcommand{\hlsms}[1]{{\sethlcolor{green}\hl{#1}}}
\newcommand\fat[1]{\textcolor{black}{#1}}

%ESSE É UM BACKUP \begin{document}
\bstctlcite{IEEEexample:BSTcontrol}

%LoRaWAN MAC layer protocol for DtS-IoT Networks
%Non-orthogonal LoRaWAN protocol for LEO Satellites-based Networks.
\title{Non-Orthogonal Multiple Access Schemes for LoRaWAN Direct-to-Satellite Networks} %in Beyond 5G Systems}MAC Direct-LoRa-Satellite (D$\textrm{Lo}$S) strategy for Internet of Space Things
\author{Felipe Augusto Tondo, Jean Michel de Souza Sant'Ana, Samuel Montejo-Sánches, Onel Luis Alcaraz López, Sandra Céspedes and Richard Demo Souza
\thanks{Felipe Augusto Tondo and Richard Demo Souza are with the Federal University of Santa Catarina, Florianópolis, SC, Brazil. \{fatondo@ucs.br, richard.demo@ufsc.br\}. Samuel Montejo-Sánchez is with Programa Institucional de Fomento a la Investigación, Desarrollo e Innovación, Universidad Tecnológica Metropolitana, Santiago, Chile. \{smontejo@utem.cl\}. Onel Luis Alcaraz Lopez and Jean Michel de Souza Sant'Ana are with the Centre for Wireless Communications, University of Oulu, Finland. \{onel.alcarazlopez@oulu.fi, jean.desouzasantana@oulu.fi \}. Sandra Céspedes is with the Concordia University, Canada. \{sandra.cespedes@concordia.ca\}.  This work has been supported in Brazil by CNPq (402378/2021-0, 305021/2021-4, 401730/2022-0), Print CAPES-UFSC ``Automation 4.0'', and RNP/MCTIC (Grant 01245.010604/2020-14) 6G Mobile Communications Systems; in Chile by ANID FONDECYT Regular No. 1241977; in Finland by the Academy of Finland (6G Flagship program, Grant 346208), The Finnish Foundation for Technology Promotion and by the European Union through the Interreg Aurora project ENSURE-6G (Grant Number: 20361812).}}

\maketitle

\begin{abstract}
    Ground-to-space communication is considered an actual and relevant step towards global connectivity and future 5G enhanced and 6G Era. This paper considers a direct-to-satellite (DtS) network and assumes a successive interference cancellation (SIC) to decode received signals sent by LoRa devices. We design a system architecture considering the outage probability for Signal-to-Noise-Radio (SNR) and Signal-to-Interference Ratio (SIR) thresholds. This work introduces two novel uplink strategies for IoT devices and evaluates their performance against traditional techniques like the ALOHA protocol. Firstly, we propose the non-orthogonal Fixed-IoT Transmission Power (FTP) strategy, where IoT messages are planned to achieve a targeted received power level at the gateway, with collision messages potentially being fixed onboard the satellite. To simulate a realistic DtS scenario, this paper defines two received levels based on SIR and capture probability, considering each elevation angle in the presence of interfering signal. Additionally, we introduce the non-orthogonal Controlled-IoT Transmission Power (CTP) scheme, allowing each device to adjust its power level within any visible time window. Simulation results, using standard link-budget parameters, demonstrate improved consistency with the FTP policy, resulting in $10\%$ fewer collisions for a payload size of $51$ bytes and a $34\%$ increase in the average number of successful uplinks for a payload size of $20$ bytes. The CTP strategy exhibits superior energy efficiency compared to FTP and ALOHA, particularly for longer payload size.
\end{abstract}

\begin{IEEEkeywords}
DtS, SIC, SNR, SIR, ALOHA, FTP, CTP.
\end{IEEEkeywords}


\IEEEpeerreviewmaketitle


\section{Introduction}

\IEEEPARstart{C}ontemporary life imposes dynamic demands and presents an extraordinary challenge to upcoming wireless communication systems. From the inception of the 1st generation (1G) to the current era of the fifth generation (5G) systems, researchers and industry have played fundamental roles in providing connectivity, overcoming barriers, and achieving unprecedented levels of performance and Quality of Service (QoS). However, a groundbreaking milestone was recently reached as the number of connected devices surpassed that of connected humans~\cite{IBM_EoT.23}. This notable advancement opens up a new opportunity for the so-called Economy of Things (EoT), providing a diversity of applications with nearly 30 billion connected Internet of Things (IoT) devices. Such astonishing number of connected devices poses a challenge to the upcoming sixth generation (6G) of wireless communication systems.


\fat{To support the massive access of a large number of devices in applications such as smart cities, smart factories, and ground logistics, the development of massive machine-type communication (mMTC) has been introduced over the years as a crucial step to provide ubiquitous connectivity on a global scale~\cite{Choi_GF_NOMA.22}. Unfortunately, applications in remote and challenging-to-access areas, such as terrestrial climate monitoring, flora, fauna, and maritime logistics, encounter substantial communication infrastructure deficits. Addressing these challenges calls for the implementation of concepts from non-terrestrial networks (NTN), employing long-range technologies to establish global connectivity for IoT applications\cite{Hirley_DtS.23,Kodheli.21_survey_Sat5G}. The upcoming 6G systems aim to integrate all non-terrestrial elements, such as satellites, unmanned aerial vehicles, diversification of access points, and gateways from other technologies, including the deployment of  High Altitude Platform Stations (HAPS)~\cite{Vic.23}. This integration needs to be carefully designed to harmoniously and effectively unify the physical, biological, and virtual worlds.}

\textcolor{black}%{In~\cite{Kodheli.21_survey_Sat5G}, the authors explore realistic application cases for satellite integration into 5G networks: (a) eMBB group, satellites can play a paramount role in extending 5G connectivity to remote areas without terrestrial infrastructure. They can bolster services through hybrid broadband networks, ensuring global coverage; (b) mMTC group, even low device complexity, satellites play a fundamental role in load balancing the IoT network, especially in cases where the terrestrial network fails natural support; (c) uRLLC group, is critical for satellite utilization and potentially serving a secondary or complementary role, due to the strict parameters of availability ($\simeq 99.99\%$), latency ($<1\%$), and packet loss ($0.001\%$).}

%\textcolor{red}{Transição ruim aqui (cel-->LPWAN)}
Low Power Wide Area Networks (LPWAN) emerge as a notable component~\cite{Georgiou.17} among terrestrial technologies for wireless communication with the capabilities to seamlessly connect ground-based devices to space. The low power consumption, long-range distances, and minimal infrastructure requirements of LPWANs make them highly attractive for direct-to-satellite IoT (DtS-IoT) applications. In this context, technology solutions like LoRaWAN~\cite{LoRa_Alianc}, SigFox~\cite{SigFox}, and NB-IoT~\cite{Capez_Fraire.22} are the most prominent examples and consistently progressed over the years. \textcolor{black}{In this sense, Lacuna Space is a pioneering player in direct-to-satellite LoRaWAN networks, while it recently expanded its constellation coverage with the launch of Lacuna Space $2$nd-Gen, hosted on NanoAvionics modular satellite platform and launched on the Space-X Transporter$-7$~\cite{Lacuna_SpaceXF9.23}.} Moreover, despite its low latency and high throughput levels, NB-IoT presents strong issues for DtS-IoT, such as increased power consumption, relatively higher cost (licensed spectrum bands), and lower battery life. Unfortunately, SigFox offers cost-effectiveness and simplicity but low data rates and a fixed packet data model~\cite{Jung2022}, while the authors are unaware of any commercial deployment of SigFox technology onboard a satellite. 

%Startups such as BehrTech and ResIOT~\cite{Behrtech,Resiot} have introduced commercial smart industry solutions. 



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[!t]
%\centering
\caption{List of Acronyms.}
\label{tab:listanom}
\begin{tabular}{ll}
\hline
\textbf{Acronyms} & \textbf{Meaning}                                        \\ \hline
CRDCA     & Contention Resolution Diversity Slotted ALOHA                                     \\
CTP      & Control-IoT Transmission Power \\
CSI      & Channel state estimation \\
DtS      & Direct-to-satellite                       \\
D2D      & Device-to-device \\
eMBB     & Enhanced mobile broadband  \\
FTP      & Fixed-IoT Transmission Power  \hspace{3cm}  \\
GW       & Gateway                     \\
IoT      & Internet of things                                               \\
LEO      & Low Earth orbit                                                  \\
LR-FHSS  & Long-range frequency hopping spread spectrum \\
HAPS      & High altitude platforms station                                       \\
%MTP      & Maximum Transmission Point \\
mMTC      & Massive machine-type Communication  \\
LPWAN    & Low power wide area networking                     \\
UAV      & Unmanned aerial vehicle \\ 
EoT      & Economy of Things \\
NOMA     & Non-orthogonal multiple access \\
NTN      & Non-terrestrial network  \\
LoS      & Line of sight                                                    \\
MAC      & Medium access control                                            \\
MTC      & Machine-type communication                                       \\
NB-IoT   & Narrowband–Internet of Things                                    \\ 
OMA      & Orthogonal multiple access                                       \\
SF       & Spread factor \\
SNR      & Signal-to-Noise Ratio\\
SIC      & Successive interference cancellation\\
RSMA      & Rate splitting multiple access \\
SIR      & Signal-to-interference ratio\\ 
URLLC      & Ultra-reliable and low-latency communications\\  \hline
\end{tabular}
\end{table}





% \usepackage{tabularray}
\begin{table*}
\caption{Review of the state-of-art for LEO satellites-based networks.}
\label{Tab:related_works}
\centering
\begin{tblr}{
  row{1} = {c},
  cell{2}{1} = {c},
  cell{2}{2} = {c},
  cell{2}{3} = {r=3}{c},
  cell{2}{5} = {c},
  cell{2}{6} = {c},
  cell{3}{1} = {c},
  cell{3}{2} = {c},
  cell{3}{5} = {c},
  cell{3}{6} = {c},
  cell{4}{1} = {c},
  cell{4}{2} = {c},
  cell{4}{5} = {c},
  cell{4}{6} = {c},
  cell{5}{1} = {c},
  cell{5}{2} = {c},
  cell{5}{3} = {c},
  cell{5}{5} = {c},
  cell{5}{6} = {c},
  cell{6}{1} = {c},
  cell{6}{2} = {c},
  cell{6}{3} = {c},
  cell{6}{5} = {c},
  cell{6}{6} = {c},
  cell{7}{1} = {c},
  cell{7}{2} = {c},
  cell{7}{3} = {r=2}{c},
  cell{7}{5} = {c},
  cell{7}{6} = {c},
  cell{8}{1} = {c},
  cell{8}{2} = {c},
  cell{8}{5} = {c},
  cell{8}{6} = {c},
  vlines,
  hline{1-2,5-7,9} = {-}{},
  hline{3-4,8} = {1-2,4-6}{},
}
{[}REF] & Technology & Protocol                   & Distinct characteristic                                                                                                                                                                                  & Channel Model                                                & SIC$^1$ \\
{\cite{Alonso.23} }  &  LoRa/LoRaWAN    & {ALOHA \\Based \\Protocol} & {End devices are configured with additional information about the satellite \\ trajectory. LoRa frames carry the same payload of 20 bytes. }       & Rician distribution                                          &  \tikzcmark       \\
{ \cite{Alvarez.22} }  & { LoRa/LoRaWAN \\ LR-FHSS}  &   & {The trajectory based policies can duplicate the amount of IoT nodes, \\  while specific variants can further boost the scalability of LPWANs.}  & Free space losses     & {\\ \tikzcmark \\}      \\ \cite{Jung.23}      & { LoRa/LoRaWAN \\ LR-FHSS}         &                & {A novel transceiver design for LR-FHSS-based DtS-IoT systems. \\ Modifying the regular LoRaWAN preamble with a new time-on-air (ToA)  \\ the work achieved 3120 frequency-hopping channels in LR-FHSS.} & {Doppler effect\\ symbol timing offset\\ co-channel interf.} & {\\ \tikzxmark \tikzxmark \\}      \\
{ \cite{Jean.24} }      & { LR-FHSS }             & {\\ ACRDA \\}           & {The ACRDA protocol is adapted to the LR-FHSS specifications, but here \\ without additional  requirements for terrestrial devices. Modifications are \\ restricted to the gateway side only.}           & { Pilot signal \\ estimation}                                      & {\\ \tikzcmark \\} \\
{ \cite{Ortigueira.21} }   & { LR-FHSS }         &  {\\ CSMA \\ }                       & { REserve-and-Send Sift-IoT (RESS-IoT) MAC protocol was proposed \\ to improve energy efficiency, throughput and fairness.  }      & { Ideal channel \\ conditions   }                            & {\\ \tikzxmark \tikzxmark \\}      \\
{  \cite{Qifan.23} }      & {Not \\ evaluated}            & {\\ NOMA \\}                      & {Multiple services (mMTC, e-MBB and MCC) coexistence for a dual-layer \\ LEO constellations.}  & {Log-normal\\ Free space losses}                             & {\\ \tikzcmark \\}      \\
{  \cite{Gao.21} }      & {Not \\ evaluated}          &                            & {A cooperative scheme is implemented for device-to-device transmission, \\ leveraging the OMA strategy to intelligently select transmission power \\ levels for both distant and nearby IoT devices.}    & {Rayleigh\\ Free space losses}            & {\\ \tikzcmark \\}      
\end{tblr}
\begin{tablenotes}
       \item [1] $^1$ We assume the follow symbols according \tikzcmark-SIC and [\tikzxmark \tikzxmark]-Not evaluated.
\end{tablenotes}
\end{table*}

    
%& I                  & \multicolumn{2}{c|}{\textcolor{red}{Falta completar}}                    & \textcolor{red}{Falta completar}           & \tikzxmark \tikzxmark             & \cite{Ortigueira.21}         \\ \cline{2-7}


%\fat{Acknowledging the demand for research studies addressing the central aspects of implementing uplink mechanisms in DtS-IoT scenarios, the following contributions of this work are elucidated below:}
%\begin{itemize} 
 %   \item Motivated by new insights, we propose a second scheme called Direct-LoRa-Satellite Non-Orthogonal Multiple Access (DLoS-NOMA). In this scheme, we strategically design IoI devices to generate pre-defined power levels received at the LEO satellite. We announced a notable enhancement in the number of successfully decoded transmissions compared to classical policies like ALOHA. 
%\end{itemize}




%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
The imminent era of smart devices, mixed with the exponential growth in data generation (expected to reach zeta-bytes), promises a lucrative scenario awaiting novel discoveries within global connectivity. Furthermore, fundamental aspects of the forthcoming 6G, such as low latency and ubiquitous wireless connectivity, are presently under discussion, offering the prospect of a significant transformation in data collection, sharing, and real-time analysis~\cite{Oulu_whiteP.20,CWC2024changing}. DtS-IoT takes the leadership in leveraging cutting-edge from the most attractive non-terrestrial technologies by installing the gateway onboard the LEO satellite, eliminating infrastructure costs. However, the trajectory dynamics, channel instability, and multi-path losses require further investigation and improvements~\cite{Fraire.survey.22}. Despite the constant speed of a Low Earth Orbit (LEO) (approximately 7 km/s)~\cite{Fraire.survey.22}, the changing number of served devices becomes a crucial discussion. In this context, Medium Access Control (MAC) directly influences system performance, becoming essential, especially in massive IoT scenarios such as mMTC (massive Machine Type Communication).


%\fat{In practice, each IoT device has a limited potential visibility time and satellite distances during the uplink phase. One satellite lap typically lasts between $3$ to $10$ minutes \cite{Fraire.survey.22}. As the network scales, more collisions are detected in received signals due to simultaneous transmission opportunities. This work focuses on a non-terrestrial network where IoT devices utilizing LoRa technology need to transmit messages to the gateway orbiting onboard a Low Earth Orbit (LEO) satellite. Similar to the approach used in~\cite{Alonso.23}, our IoT devices are equipped with additional information about the satellite's trajectory. After an initial step, which may occur during the setup phase, each user becomes aware of the visibility times. \textcolor{red}{Muitas infos do system model, rever aqui..}Following the authors in~\cite{Corazza.94}, we model the channel fading as a combination of Rice and log-normal random processes, with the multipath parameters statistically validated considering the respective range of elevation angles through practical environment measurements. Additionally, the path loss assumes the Friis transmission equation. Finally, we also consider the exact location of IoT devices, as well as, the visibility time window during the satellite lap over a selected target area}


Built upon ALOHA-based protocol, LoRaWAN may struggle under heavy traffic. Similar to terrestrial networks, a large number of IoT devices within the satellite footprint may generate a considerable number of collisions, leading to several issues in terms of scalability and energy efficiency~\cite{Ortigueira.21,Georgiou.17}. Nevertheless, when two LoRa devices transmit simultaneously, the receiver can often recover one of the overlapping signals, the so called capture effect. Moreover, by removing one of the colliding signals, it could be possible to recover the other one as well. However, resolving these collisions requires identifying signal characteristics such as differences in power and timing~\cite{Xiao.22}. Enhancing the scalability of LoRa satellite networks, it is essential to investigate new MAC protocols towards massive connectivity. In practice, the satellite lap typically lasts $3$ to $10$ minutes, offering a limited visible time window to the IoT device transmissions~\cite{Fraire.survey.22}. Our focus is concentrated on a direct-to-satellite scenario, where the IoT devices utilize LoRa/LoRaWAN technology to transmit messages to the gateway orbiting onboard the LEO satellite.

%\textcolor{red}{Antes de abordar o related works, faltou abordar um problema....MAC protocols that could be suitable for LoRa-based DtS-IoT networks...improve uplink scalability, energy consuption..}

\subsection{Related Works}


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Since the announcement in~\cite{LR-FHSS_annou}, LoRa Alliance has expanded the guidelines of LoRaWAN protocol for LPWANs with the Long-range frequency hopping spread spectrum (LR-FHSS) technology. The new physical layer is designed to address satellite IoT services and improve the capacity for terrestrial LoRaWAN networks~\cite{Boquet.21}. Recent years have seen noteworthy advancements towards new perspectives, especially the feasibility of LR-FHSS to support dense networks~\cite{Asad.LR-FHSS.22}. Some fundamental baselines for the LoRaWAN LR-FHSS modulation-coding scheme were introduced by Asad et al.~\cite{Asad.LR-FHSS.22}, where it is shown that a LEO satellite with Iridium characteristics can serve $50$ thousand devices. %Through average probability of packet delivery, headers success probability, and probability of enough payload fragments reception the simulated results are suitable for DtS, but However, the authors highlight that technical information should be re-validated including the experimental testbed.}



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

A new design was proposed by~\cite{Maleki.23} for the device-to-device (D2D) strategy, incorporating LR-FHSS technology in satellite communication links. While the D2D-link scenario may not be favorable in this system, the study demonstrated significant potential advancements for dense IoT networks. Nevertheless, several limitations, such as the reliance on a distance threshold for establishing communication between devices and the challenges of managing energy and signal propagation effects to maintain synchronization between pairs, pose obstacles to practical implementations. %talvez um modo híbrido possa ser pensado para que quando o tenha poucos devices na rede, o sistema atue como um ALOHA por exemplo.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

Motivated by the performance achieved with medium access schemes that devices are adapted to transmit message replicas using slotted ALOHA, the so-called Contention Resolution Diversity Slotted ALOHA (CRDSA) was recently proposed in~\cite{Jean.24}. In this study, the authors adapted the asynchronous contention resolution-aided ALOHA (ACRDA) protocol to improve the performance parameters such as average network success, goodput, and reliability level in the long-range frequency hopping spread spectrum (LR-FHSS) technology. While the simulation results are promising, the authors introduce a capture effect threshold in LR-FHSS that does not guarantee robust references in the current literature. %\cite{Knop.LR-FHSS.24}.
Recently, LR-FHSS has attracted a lot of attention as a promising technology for upcoming satellite-based networks~\cite{Boquet.21,Jean.24,Knop.LR-FHSS.24,Maleki.23,Asad.LR-FHSS.22}. However, it still lacks in-depth investigations into the dynamic influences of direct-to-satellite transmission. Even though potentially promising in reliability and energy efficiency, LR-FHSS technology is currently in testing progress, as reported in the partnership between Semtech and Lacuna Space~\cite{Semtech_Lacuna.22}.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

To expand the boundaries in LoRa technology for satellite communication systems, an attractive research direction is to allow the network's operation always under the most optimal with low energy consumption and complexity. In \cite{Alonso.23}, the authors investigate a LoRa-based DtS-IoT assuming the Friis model for the propagation path loss and Rician distribution for channel fading. In addition, the gateway is installed on-board the satellite and only one uplink transmission is allowed per device. They propose to modify the traditional ALOHA protocol for IoT devices by dynamically adjusting their transmission rates according to the optimal network conditions. Furthermore, the novel protocol assumes that the devices are configured with extra information about the satellite trajectory, i.e., each node has acknowledgment of the available times of the gateway.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Contributing with extensive studies on the link budget for LoRa in a direct-to-satellite scenario, the authors in~\cite{Hirley_DtS.23} evaluating the impacts caused by the Doppler effect on the reliability of the LoRa link. The satellite speed is dynamic throughout coverage, so the work demonstrates through parameters such as packet loss and Doppler rates that the results improve packet delivery in $82\%$ for the most vulnerable spread factor (SF12) when using LoRa parameters such as 125 kHz bandwidth, 433 MHz carrier frequency and 59 bytes of payload. In the same study, the authors reported that bandwidth, carrier frequency, and selection of SFs significantly impact the performance of DtS links. The study also highlight that spread factors represent a moderate influence on the network performance.



%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%


Similar to terrestrial networks, the non-orthogonal multiple access (NOMA) power domain is employed in earth-satellite links to enhance the system's reliability and spectral efficiency, especially when a massive quantity of devices need to be connected~\cite{Liu.21_NOMA6G}. Notably, significant progress in exploring NOMA through numerous studies~\cite{Qifan.23,Gao.21,PD_NOMA_SAT.YAN.19,PD_NOMAchen2023signal} has strategically enabled transmission on the device side and facilitated the implementation of successive interference cancellation (SIC) at the satellite receiver. In ~\cite{Gao.21}, a cooperative NOMA (C-NOMA)-assisted hybrid satellite-terrestrial networks (HSTN) was considered, where a relay and the strong user cooperate to forward information. Other authors in~\cite{BoZhao.22} presented the joint NOMA clustering and power allocation in IoRT for DtS systems.

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\textcolor{black}{Recently, Rate Splitting Multiple Access (RSMA) has emerged as a novel MAC protocol, assuming linear rate splitting at the transmitter and successive interference cancellation (SIC) at the receiver. In satellite communication systems, the RSMA approach has been investigated in studies like~\cite{Ullah.23, Li.23-RSMA}, where the authors explore a hybrid co-existing network in the downlink phase. In~\cite{Ullah.23} a primary geostationary satellite (GEO) serves ground users using orthogonal multiple access (OMA), and the LEO satellite accommodates remaining users following the RSMA protocol. The authors in~\cite{Bruno_Clerckx.23} clarify the benefits of splitting messages strategy.} %However, as indicated by~\cite{Mao.22-RSMA-Survey}, the number of SIC layers increases exponentially with the number of users. This exponential growth imposes significant complexity on the receiver side.} 
%\textcolor{black}{While studies investigate RSMA-based IoT links via satellite, the largest share focuses on the downlink phase~\cite{Ullah.23,Cui_Clerckx.23_sat_downli,Yin_Clerckx.23_sat_downli}. Moreover, the RSMA uplink schemes in DtS-IoT scenarios require further improvements considering dynamic effects and excessive signaling~\cite{Mao.22-RSMA-Survey}. As users split their messages, it becomes necessary to establish splitting rate requirements for both transmitters and receivers. Additional signaling is a relevant issue and fundamental to ensure the synchronization of such knowledge.}


\subsection{Paper Contributions}
This work introduces two innovative multiple access schemes for LoRaWAN direct-to-satellite networks. As shown in Table.~\ref{Tab:related_works}, non-orthogonal schemes have improved the uplink scalability in LoRa-based systems. Nevertheless, research efforts such as those by~\cite{BoZhao.22} may face challenges due to computational complexity in identifying the optimal solution proposed. More recently, [Wang] already considers the use of NOMA in networks with more than one layer of satellites, which from a practical point of view requires a high implementation investment cost. Despite the significant advancements achieved by~\cite{Gao.21} in optimizing completion time in cooperative networks using NOMA, we need to consider numerous complications parameters such as distance, device coordination, and most importantly, dynamics of the satellite orbit. 

Different from ALOHA variant protocols used in~\cite{Alonso.23},  we strategically plan IoT device transmissions to generate a predetermined power level at the LEO gateway. Furthermore, we propose MAC policies considering the Signal-to-Interference ratio (SIR) and the capture probability: (a)- first, the so-called FTP policy assumes that an IoT device generates a pre-designed average received power level at the satellite, using a fixed transmission power; (b)- using power control, in CTP each device can select a random visible time and adjust its transmission power according to the average received power level to be seem at the satellite. Applying Successive Interference Cancellation (SIC), we evaluate the trade-off between the average number of successfully decoded transmissions and energy consumption. The simulation results illustrate that employing FTP leads to a $10\%$ reduction in collision messages and an added $34\%$ increase in the average number of successfully decoded packets. Notably, for longer payload sizes, CTP outperforms FTP and the regular ALOHA protocol in terms of energy efficiency.

%\textcolor{red}{The following section provides an overview of the expectations in DtS-IoT, specifically focusing on the latest advancements in MAC protocols for satellite-based IoT applications.}

The rest of this paper is organized as follows. Section II describes the system model, while Section III formulates the proposed direct-to-satellite power schemes. Section IV presents the simulation parameters, while Section V discusses the numerical results. Finally, Section VII concludes the paper and briefly discusses future works.


\section{System Model}
\label{Sec:system_model}

\fat{We consider an IoT device network uniformly distributed within the target area within the coverage of a Low Earth Orbit (LEO) satellite. Inspired by previous works such as~\cite{Alvarez.22, Alonso.23}, we assume that IoT devices use LoRa technology to transmit data packets to the satellite in orbit. Fig.~\ref{fig:System_Model} shows the system architecture, where IoT applications are deployed on the ground and communicate with a gateway on board the LEO satellite. Meanwhile, a terrestrial backhaul is composed of a ground station that is responsible for receiving the packets from the satellite and forwards them to a network server (NS).}


\begin{figure}[!t]
    \centering
    \includegraphics[width=1\columnwidth]{figuras/SYS_OP_II.PNG}
    \caption{The DtS-IoT system architecture, composed of a gateway on-board the LEO satellite, IoT applications spread over the target area, and the terrestrial backhaul.} 
    \label{fig:System_Model}
\end{figure}


\textcolor{black}{We describe the total number of satellite laps as $J$ and the total number of IoT devices as $U$. Each IoT device experiences distinct visibility periods, offering different opportunities for uplink transmissions. Furthermore, the total window duration time is determined by the interval $\mathcal{T}_{j,u}=\left [\ O_{j,u} , F_{j,u} \right ]$, where rise-time $O_{j,u}$ and set time $F_{j,u}$ for $j\in \left \{ 1,2,...,J \right \}$ and $u\in \left \{ 1,2,...,U \right \}$, denotes the instants that the IoT device appears and disappears from the satellite footprint. Considering a $j$ lap, we define $\mathbb{T}_j\textrm{}=\left \{ \mathcal{T}_{j,u},...\mathcal{T}_{j,u} \right \}$ as the set of all visible times.
%Note that, between the initial visible time and set-time (both occurred in the minimum elevation angle $\alpha^{min}_{j,u}$, in degrees), we also describe the maximum elevation angle as $\alpha^{pk}_{j,u}$, i.e., the peak of LEO trajectory achieved in the minimum satellite distance.
The initial visible and set times occur with minimum elevation angle $\alpha^{min}_{j,u}$, while the peak of the LEO trajectory occurs with maximum elevation angle $\alpha^{pk}_{j,u}$, both in degrees.
For our initial analysis, \textcolor{black}{we assume that each IoT device $u$ transmits in the satellite lap $j$ following the ALOHA protocol, using the same bandwidth $B$ and fixed transmission power $Pt_{j,u}$}. However, the uplink phase only occurs during $\mathcal{T}_{j,u}$ interval. 
%We assume that the initiation of the coverage cycle can be signaled through a beacon from the LEO satellite~\cite{Alvarez.22,Alonso.23}.
We assume that the LEO satellites constantly broadcast beacons to notify devices about gateways in coverage.
Finally, to ensure that the transmitted messages reaches the gateway (GW) with sufficient power, the IoT devices are configured to use a robust spreading factor $SF=12$ and bandwidth $B=125$ kHz. Note that, the specific required spreading factor or bandwidth may depend on the orbit height and target area, as indicated in~\cite{TTN_Mod_Rate.21}.}



\fat{The signal sent by each LoRa device is received at the LEO gateway under different channel conditions and influences relatives to the respective elevation angle $\alpha$. Analysing a reference IoT device transmission ($u=1$), the received signal can be expressed as the sum of the attenuation of the transmitted signal, interference, and noise, as follows:} 
%
%
%\begin{equation}
%   r=\sqrt{P_t g_1(\alpha_0)} h_1 s_1 +\sum_{k=2}^{\mathcal{N}} \sqrt{P_t g_k(\alpha_k)} h_k s_k + w,
%\end{equation}
%
\begin{equation}
 r_{j,1}(\alpha)\!=\!\sqrt{\mathcal{P}g_{j,1}(\alpha_{j,1})} h_{j,1} s_{j,1} + \sum_{u=2}^{U} \! \sqrt{\mathcal{P} g_{j,1}(\alpha_{j,u})} h_{j,u} s_{j,u} + w,
\end{equation}
%
%
\fat{where $\mathcal{P}={Pt}_{j,u}G_{t}G_{r}$ represents the transmitted power, and respectively, transmitter’s and receiver’s antenna gains, $g(\cdot)$ is the path loss as a function of the elevation angle $\alpha$, $h$ is the channel fading gain, $s$ is the modulated signal and $w$ is the additive white Gaussian noise (AWGN) with zero mean and variance $\sigma^{2}_w=-174+\mathsf{NF}+10\log_{10}B=-117$ dBm, with the receive noise figure $\mathsf{NF}=6$ dB~\cite{semtech2015an1200}.}
%We denote the path loss of the $u$-th device as a function of the elevation angle by $g_{j,u}(\alpha_{j,u})$; the $u$-th fading channel gain is represented by $h_{j,u}$ and modulated signal is assumed as $s_{j,u}$. Furthermore, we consider $w$ as additive white Gaussian noise (AWGN) with zero mean and variance $\sigma^{2}_w=-174+\mathsf{NF}+10\log_{10}B=-117$ dBm, with the receive noise figure $\mathsf{NF}=6$ dB~\cite{semtech2015an1200}. The section ends with more channel fading and path loss details.}

\begin{table}[!t]
\caption{Non-terrestrial channel fading parameters.}
\label{Tab:fading_parameters}
\centering
\begin{tabular}{ccc}
\hline
\multicolumn{3}{c}{Parameters $K \mu \sigma$ for proposed channel model and elevation angle $\alpha$} \cite{Corazza.94}         \\ \hline
\multicolumn{1}{c|}{$K(\alpha)$}                           & \multicolumn{1}{c|}{$\mu(\alpha)$}      & $\sigma(\alpha)$              \\ \hline
\multicolumn{1}{c|}{$K_{0} + K_{1}\alpha+K_{2}\alpha^{2}$} & \multicolumn{1}{c|}{$\mu_{0} + \mu_{1}\alpha + \mu_{2}\alpha^{2}+ \mu_{3}\alpha^{3}$} & $\sigma_{0}+\sigma_{1}\alpha$ \\ \hline
\multicolumn{3}{c}{Coefficients for empirical formulas}                \\ \hline
\multicolumn{1}{c|}{$K_0=2.731$}              & \multicolumn{1}{c|}{$\mu_0=-2.331$}                & $\sigma_0=4.5$                    \\
\multicolumn{1}{c|}{$K_1=-1.0474 \ 10^{-1}$}              & \multicolumn{1}{c|}{$\mu_1=1.142 \ 10^{-1}$}     & $\sigma_1=-0.05$                    \\
\multicolumn{1}{c|}{$K_2-1.0474 \ 10^{-1}$}              & \multicolumn{1}{c|}{$\mu_2=-1.939 \ 10^{-3}$}     &         \\
\multicolumn{1}{c|}{}                   & \multicolumn{1}{c|}{$\mu_3=-1.094 \ 10^{-5}$}                      &                               \\ \hline
\end{tabular}
\end{table}

\subsection{Non-terrestrial channel fading}

\fat{
%Like terrestrial communication systems, the received signal power in DtS-IoT varies randomly over distance or time as a function of shadowing and/or multipath fading~\cite{Goldsmith_2005}.
Due to the non-geostationary orbit, the elevation angle $\alpha$ changes with time, modifying the relative channel conditions. There are available models such as Loo and Nakagami-m distributions that can be used to characterize the fading gain, but traditional works as~\cite{Choi_GF_NOMA.22,Corazza.94, Salamanca.19} mention that Rice fading is an attractive approach for the general situation and widely applied to make accurate performance estimates, especially for ground-to-space links. \textcolor{black}{Like the authors in~\cite{Corazza.94, Alonso.23}, we model the received  complex fading envelope $h$ as a combination of two process. The $z$ is assumed as a Rice component, while $\mathcal{S}$ contribution modeled as Log-normal distributed. Thus, the received signal envelope $h$ have the probability density function (PDF) described as~\cite{Corazza.94}:}}
%
\begin{equation}
    f_h(h)=\int_{0}^{\infty} f(h|\mathcal{S}) f_{\mathcal{S}}(\mathcal{S})
\label{eq:overall_RxL}
\end{equation}
%
\textcolor{black}{In (\ref{eq:overall_RxL}), $f(h|\mathcal{S})$ indicates the Rice PDF specified according to the shadowing $\mathcal{S}$ by the equation~\cite{Corazza.94}:}
%
\begin{align}
    f(h|\mathcal{S}) &=\frac{h}{\sigma^{2}\mathcal{S}^{2}}  \mathrm{exp} \left[-\frac{1}{2} \left ( \frac{h^{2}}{\mathcal{S}^{2}\sigma^{2}}+2K \right ) \right] \nonumber \\
    &\centerdot \ \ I_o\left( \frac{h}{\mathcal{S}\sigma}\sqrt{2K} \right),
\end{align}
%
\fat{where, $\sigma^{2}=1/2(K+1)$, $I_o$ is the zero-order modified Bessel function while $K$ represents the Rice factor, which means the ratio between the power in the line-of-sight (LOS) component and that without line components (NLOS). The higher $K$, the greater the contributions establishing received power variability around the mean value. Our model also assumes the log-normal shadowing, $S$ with the probability density function represented by~\cite{Corazza.94}:}
\begin{equation}
    f_{\mathcal{S}}(\mathcal{S}) = \frac{1}{\beta \sigma \mathcal{S} \sqrt{2\pi}} \mathrm{exp}\left [ -\frac{1}{2} \left ( \frac{\mathrm{ln} \ S - \mu}{\beta \sigma} \right )^{2} \right ].
\end{equation}

\fat{Motivated by statistical model for land mobile satellite channels proposed in~\cite{Corazza.94}, we assume the mean and variance associated of the normal variate as $\mu$ and $(\beta \sigma)^{2}$, where $\beta=(\mathrm{ln} 10/20)$. Additionally, depending on the relative values of parameters $K$, $\mu$ and $\sigma$, the proposed channel model can be modify to selective or non-selective fading models. In Table~\ref{Tab:fading_parameters} we introduce the respective parameters and formulas validated for a rural tree-shadowed environment~\cite{Corazza.94}. Data fitting consider the greater $\alpha$, the smaller is $\sigma$ and the larger will be rice factor $K$, i.e, increasing LOS portion and variation of mean received power signal.}



\begin{figure}[!t]
    \centering
    \includegraphics[width=1\columnwidth]{figuras/geometry_op_II.pdf}
    \caption{The ground-space geometry described as a function of parameters such as: altitude $H$, distance $d$, elevation angle $\alpha$, radius of Earth $R_E$ for a relative visible time window.} 
    \label{fig:geometry}
\end{figure}


\subsection{Path Loss}

\fat{Before delving into the detailed path loss model, it is essential to first comprehend the geometry inherent in the satellite trajectory. In Fig.~\ref{fig:geometry}, we present a DtS-IoT link considering the mathematical baselines to calculate the distance between a deployed device and the minimal elevation angle $\alpha_{min}$. As described for the authors in~\cite{Hirley_DtS.23,Maleki.23}, we can have:}
%-------------------
\begin{align}
    d(\alpha)&=\left [ \sqrt{\left ( R_{E}\!+\!H \right )^{2}-(R_{E} \cos(\alpha ))^{2}} - R_{E} \sin(\alpha ) \right ] \\
  \alpha(d)&=\sin^{-1}\left ( \frac{H^{2}+2HR-d^{2}}{2dR} \right ).
\end{align}
%-------------------


For the sequential equations, $R_E=6378 km$ corresponds to the radius of the Earth, while $H$ is the orbital height of the LEO satellite. For practical considerations, at the beginning of the visible time window, Fig.~\ref{fig:geometry} also shows the minimal elevation angle assumed as $\alpha^{min}$. Additionally, we consider that during a satellite lap $j$, the IoT device $u$ can transmit its message at any visible time with the elevation angle defined as $\alpha_{j,u}$, for $\alpha \in \left \{ \alpha^{min}_{j,u},...,\alpha^{pk}_{j,u} \right \}$. By simplifying the satellite orbit, IoT devices are constrained to three crucial elevation angles and two phases within the time window to transmit their messages: first, the ascendant phase goes from minimum to maximum elevation angle $\left ( \alpha^{min}\rightarrow \alpha^{pk} \right )$, while the descendent phase is composed by the opposite order.


\fat{We model the path loss using the Free space transmission formula as a function of each elevation angle. The distance from ground devices to satellite is assumed  in meters. Due to the region parameters, we highlight that the frequency value depends of the coverage target area configured according to the LoRa requirements~\cite{LoRa_Alianc}. Finally, the large-scale propagation effect can be modeled (in dBm) as:}
\begin{equation}
    g_{j,u}(\alpha_{j,u}) = 20\log_{10}\left ( \frac{\lambda}{4\pi d(\alpha_{j,u})} \right ),
\end{equation}
where $\lambda=c/f_{req}$ represents the wavelength, $c=3 \times 10^{8}m/s$ is the speed of light and $f_{req}$ (in MHz) is the carrier frequency.




\subsection{DtS outage probability analysis}

\fat{The minimum Signal-to-Noise Ratio (SNR)  required for reliable packet decoding can be specified for particular technologies. Considering the LoRa-to-space signals, we need to discuss the conditions under which the receiver can successfully demodulate IoT messages in the gateway, as well as the parameter influences leading to outage events.} 

\fat{Firstly, the connection probability depends on the selected elevation angle $\alpha$, the distance between the device and gateway, fading gain, and path loss. In collision-free scenarios, a device $u$ can establish a connection with the LEO GW with $\Phi_n$ probability. On the other hand, we define that a collision probability $\Theta_n$ occurs when multiple devices transmit simultaneously, and the Signal-to-Interference Ratio (SIR) falls below a predefined threshold. Moreover, note that two different conditions about thresholds are supported due to the capabilities of LoRa technology: working with the signal-to-noise sensitivity ratio and/or capture effect property with interference.}

In this context, we assume the outage conditions like the authors in \cite{Arliones.18,Jean.20,Maleki.23,Alonso.23} as follows:

\vspace{0.2cm}


\textbf{Definition 1. \textit{Connection mode}} \textit{If the Signal-to-Noise Ratio (SNR) of the received signal is lower than a reception threshold $\gamma$, the IoT device is assigned as not connected to the gateway. This threshold is established to guarantee successful signal detection without interference. Considering LoRa uplink, variations in terms of packet size, bandwidth $B$, and spreading factor $SF$ contribute to distinct reception sensitivities at the gateway. Moreover, the connection probability can be expressed by $u^{th}$ device in $j$ lap:}

\begin{align}
    \Phi_{j,u}(\alpha)&=\mathrm{Pr}\left \{\frac{ |h_{j,u}|^2 \mathcal{P}g_{j,u}(\alpha_{j,u})}{\sigma_{w}^2} \geq \gamma \bigg| {g_{j,u}(\alpha_{j,u})} \right \} \nonumber \\
%    &= \mathrm{Pr}\left \{ |h_{j,u}|^2 \geq \frac{\sigma_w^2 \gamma}{\mathcal{P} {g_{j,u}(\alpha_{j,u})}} \bigg|   {g_{j,u}(\alpha_{j,u})} \right \} \nonumber \\ %= \textrm{exp}\left ( - \frac{\sigma_w^2 \gamma}{\mathcal{P} g_1(\alpha)} \right ) 
%    &=\int_{0}^{\frac{\sigma_w^2 \gamma}{\mathcal{P} {g_{j,u}(\alpha_{j,u})}}} f_h(h) {dh}     \nonumber   \\
%                        &=\frac{1}{\beta\sqrt{2\pi}}\int_{0}^{\frac{\sigma_w^2 \gamma}{\mathcal{P} {g_{j,u}(\alpha_{j,u})}}} \left ( \frac{C\sqrt{C}}{z^2} \right ) \nonumber \\
%                        & \centerdot \textrm{exp}\left \{ -\frac{1}{2}\left [ \left ( \frac{1}{C}\!-\!K \right )+y^2 \right ] \right \}I_o\left ( \sqrt{2K}\sqrt{C} \right ){dh},
    \label{Eq:Connec_prob}
\end{align}

where in (\ref{Eq:Connec_prob}), the term $C=z^2/\left ( {\mathcal{S}^{2}\sigma^{2}} \right )$ and $y^2$ as $\left [ \left ( \mathrm{ln} \ S - \mu \right ) / \beta \sigma \right ]^{2}$.

%Using (\ref{Eq:Connec_prob}), the connection probability considering the shadowed-Rice fading is rewritten as follow:


%\begin{align}
%    _{j}^{u}\Phi(\alpha)&=\int_{0}^{\frac{\sigma^2 \gamma}{\mathcal{P} g_1(\alpha)}} f_h(h) {dh}     \nonumber   \\
%                        &=\frac{1}{\beta\sqrt{2\pi}}\int_{0}^{\frac{\sigma^2 \gamma}{\mathcal{P} g_1(\alpha)}} \left ( \frac{G\sqrt{G}}{z^2} \right ) \nonumber \\
%                        & \times \textrm{exp}\left \{ -\frac{1}{2}\left [ \left ( \frac{1}{G}-K \right )+y^2 \right ] \right \}I_o\left ( \sqrt{2K}\sqrt{G} \right )
%\end{align}


%\begin{align}
%  _{j}^{u}\Phi(\alpha)=\frac{1}{4\beta \sqrt{2\pi}} \cdot \sum_{b=0}^{\infty}\frac{1}{b!\Gamma \left ( 1+b \right )} \int_{0}^{\frac{\sigma^2 \gamma}{\mathcal{P} g_1(\alpha)}} \left ( \frac{z^{3}2K}{\mathcal{S}^{4} \sigma^{4}} \right ) \\
%  \mathrm{exp} \left [ -\frac{1}{2} \left[ \left ( \frac{z^{2}}{\mathcal{S}^{2}\sigma^{2}}+2K \right ) + \left ( \frac{\mathrm{ln} \ S - \mu}{\beta \sigma} \right )^{2} \right] \right ]
%\end{align}

\textbf{Definition 2. \textit{Collision}} \textit{We assume two collision situations: (a) when a transmitted data packet collides with one or more messages from the others devices. In this work, our devices are configured with the same spread factor $SF$; (b) secondly, we assume the capture effect using the difference between the received power of the desired signal and the sum of interference is lower than $\psi$ threshold. Similar the authors in ~\cite{Jean.20,Maleki.23}, we used the capture effect to model the outage probability in the presence of interference as: }


\begin{align}
    \Theta_{j,1}(\alpha)\!&=\!\mathrm{Pr} \!\left \{ SIR_{j,1} \geq \psi \bigg| g_{j,1}(\alpha_{j,1}),...,g_{j,u}(\alpha_{j,u}) \right \} \nonumber \\
     &=\! \mathrm{Pr} \! \left \{\! \dfrac{|h_{j,1}|^2 \mathcal{P} g_{j,1}(\alpha_{j,1})}{\sum\limits_{ u \! \in \! U}^{}\!|h_{j,u}|^2 \mathcal{P} g_{j,u}(\!\alpha_{j,u}\!)} \!\geq \!\psi \bigg| g_{j,1}(\!\alpha_{j,1}\!),.,g_{j,u}(\!\alpha_{j,u}\!)\! \right \}
     \label{Eq:prob_SIR}
\end{align}



\textcolor{black}{We explore the potential of capture effect in the  following sections using SIC procedure.}


\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{figuras/Received_Pr_2024_p_mark_March.eps}
    \caption{The received power for $U=4$ devices per lap time deployed in the country of  France. The yellow star is the maximum power, and the circles in magenta are the power levels $\mathcal{L}_1$, $\mathcal{L}_2$ for ascendant and descendent phases.} 
    \label{fig:DtS_Pr}
\end{figure}


\section{Direct-to-Satellite LoRa/LoRaWAN schemes}
\label{Sec:DtS-Schemes}

\textcolor{black}{Currently, MAC schemes in DtS-IoT aim to enhance the scalability of the ground-to-satellite link with solutions focused on LoRa/LoRaWAN~\cite{Alonso.23,Alvarez.22} technologies. As the listed works still require further investigation and improvement, here, we introduce two novel uplink strategies based on the visibility time window of each IoT device. First, the LEO satellite broadcasts a beacon to the network devices to communicate its presence. Taking into account that our IoT devices are configured with extra information about the orbit executed during the trajectory, it will be possible to randomly select or predict when a data packet transmission starts. To understand the proposed DtS-IoT MAC strategies, the received power signal is explored next.}

\textcolor{black}{\textit{Example 1: Let us to consider a \textcolor{black}{real study case of LacunaSat-3~\cite{LS3.2020} orbiting over the country of France\footnote{In Section~\ref{Sec:Summary_parameters}, we present more detailed information regarding the simulation platforms}.} where $U=4$ LoRa devices need to transmit data packets to the LEO gateway in the $j=1$ initial lap. Now, selecting LoRa/LoRaWAN parameters such as $Pt_{j,u}=14$ dBm for $u \in\left \{ 1,2,3,4 \right \}$, $G_t=0$ dBi, $G_r=13.5$ dBi, $B=125$ KHz and $f_{req}=868$ MHz, we can calculate the received power signal as a function of each lap time. Fig.~\ref{fig:DtS_Pr} shows the received power for each device (in dBm) per lap time. The yellow star represent the maximum receive power achieved in the maximum elevation angle $\alpha^{pk}_{1,u}$,  for $\alpha^{pk}_{1,1}> \alpha^{pk}_{1,3}> \alpha^{pk}_{1,2}> \alpha^{pk}_{1,4}$ .The blue line is the $1^{th}$ device to appear on the satellite footprint, then the orange line is the $2^{th}$ device, and so on. Furthermore, if the first two devices decide to transmit at the maximum received power, both signals will be received at the gateway as collision messages. Although the trade-off maximum received power and minimum distance between the ground-satellite link, the challenge problem is the high probability of devices reaching in the maximum elevation angle at the same time.}}

\textcolor{black}{Next, we introduce the uplink policy that plans IoT transmissions to generate an desired power level received at the LEO gateway and strategically contributes to decode collision messages.}




\subsection{Non-orthogonal Fixed-IoT Transmission Power (FTP)}

\textcolor{black}{Classical LoRa/LoRaWAN protocols operates with ALOHA-based policies and Class A or Class B devices. Like terrestrial networks, ALOHA MAC protocols would case a large number of collisions or needs to force the IoT device to transmit into discrete time slots. Here, as highlighted in Section~\ref{Sec:system_model}, the IoT device is aware with preliminary knowledge of the LEO trajectory and visible times. We assume the total number of possible generated power levels as $L$. Hence, a device $u$ can generate a receivable power level assumed as $\mathcal{L}_{l}$, for $l \in \left \{ 1,2,...,L \right \}$. Furthermore, we designate the power levels received in the ascending and descending orbits as $P^{l'}_{j,u}$ and $P^{l''}_{j,u}$, respectively. Note that, following Fig.~\ref{fig:DtS_Pr}, the ascending satellite trajectory goes from $\alpha^{min}_{j,u}$ to maximum elevation angle $\alpha^{pk}_{j,u}$. Meanwhile, descending orbit has the opposite sequence angles. \textcolor{black}{As mentioned by practical considerations in~\cite{PD_NOMA_SAT.YAN.19,PD_NOMAchen2023signal}, NOMA schemes perform significantly better when only two users are in a NOMA group. To avoid the device-to-device approach in DtS-IoT and to reduce additional complexity at the receiver, we plan to generate only two received power levels at the satellite gateway}. Aiming a realistic scenario, we present the non-orthogonal Fixed-IoT Transmission Power (FTP) policy adapting traditional NOMA and generate a total of $L=2$ levels into the satellite gateway as follows:}

\begin{itemize}
    \item \textbf{Case1}: The satellite receives a single packet from device $u=1$ considering the power level $\mathcal{L}_1$, defined according to the first received power, commonly for all IoT devices and transmitted at minimum elevation angle $\alpha^{min}_{j,u}$. In Fig.~\ref{fig:DtS_Pr}, the magenta circles illustrate the generated power levels in the ascendant $P^{1'}_{1,1}$ and descendant $P^{1''}_{1,1}$ directions;
    \item \textbf{Case2}: The satellite receives a single packet at power level $\mathcal{L}2$. Taking into account the LoRa capture effect, we design the second received levels $P^{2'}_{1,1}$ and $P^{2''}_{1,1}$ using the outage probability for the signal-to-interference ratio (SIR) and a threshold $\psi$. In the following section, we provide more details about the second level.  
\end{itemize}


\subsection{Non-orthogonal Controlled-IoT Transmission Power (CTP)}


Next, we proposed the second novel direct-to-satellite MAC protocol considering the power levels $\mathcal{L}_1$ and $\mathcal{L}_2$ that could arrive at the gateway at any lap time. In this scheme, the IoT devices can transmit data packets randomly and adjust/control their transmission power according to the projected power level. As we know, the closer the uplink transmission to the peak of the LEO orbit, the lower will be the adjusted transmission power. The so-called Non-Orthogonal Controlled-IoT Transmission Power (CTP) work with the proposed conditions bellow: (a)-the satellite receives a single packet in power level $\mathcal{L}_1$, but herein, the uplink transmissions are randomly decided by IoT nodes. Furthermore, each transmission power $P_t$ is adjusted according the power level; (b)-unlike the fixed transmission power strategy, here, the power $\mathcal{L}_2$ is generated according to the controlled transmission power and can be received at any given time. 



%\begin{figure}[!ht]
%    \centering
%    \includegraphics[width=\columnwidth]{figuras/Received_Pr_2024.eps}
%    \caption{Average number of uplinks for total number of device $U=200$ applying DtS-IoT schemes: DLoS-FTP, ALOHA protocol, DLoS-CTP and DLoS-MTP.} 
%    \label{fig:Th_DtS_schemes}
%\end{figure}



\subsection{Satellite SIC approach}

While some devices are benefited from favorable geographic positions, many others confront unfavorable conditions, especially in long distances or dense network situations. In general, as higher the number of total devices $U$, as the collision probability increases. In this study, we assume that not only can the strongest signal be decoded successfully for collision events, but also, through Successive Interference Cancellation (SIC), the receiver can attractively decode other collided messages. In the same direction works like~\cite{Alonso.23,Jean.24} we aiming to explore collision-related messages using SIC with strategic mechanisms for IoT device transmissions.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{figuras/SIR_2024_March.eps}
    \caption{Signal-to-Interference Ratio $SIR_{j,u}$ for the first four devices in the $j=1$ satellite lap time, considering the common power level $\mathcal{L}_{1}=-123.64$ dBm and threshold $\psi=1$ dB.} 
    \label{fig:DtS_SIR}
\end{figure}



First, using Definitions 1 and 2 we define the coverage probability as $\mathcal{R}_{j,1}(\alpha) =\left [ \Phi_{j,1}(\alpha) \Theta_{j,1}(\alpha) \right ]$, the probability that a device $u$ achieves the SNR or SIR thresholds~\cite{Aamir.19}. Thus, we can analyse a common case in LoRa/LoRaWAN networks where two collisions messages arrive at the gateway simultaneously. More specifically, the coverage probability for the reference signal considering the SIC approach can be describe as:
\begin{equation}
    \mathcal{R}_{j,1 \to SIC} =\left [ \Phi_{j,1}(\alpha) \Theta_{j,1}(\alpha) +\Phi_{j,1}(\alpha) \Theta_{j,2}(\alpha) \right ],
\end{equation}
where the second term represents the decoding of the interfering signal first, and then, by applying SIC, the reference signal should also be decoded without interference. 

We describe the probability of the interfering signal being sufficiently stronger than the reference signal, enabling it to be decoded first via the capture effect, as follows:
\begin{align}
    \Theta_{j,2}(\alpha)=&\mathrm{Pr}\left \{ \frac{P^{2'}_{j,1}}{P^{2'}_{j,1}} \geq  \psi \bigg| \left |\varphi \right |=1, g_{j,1}(\alpha) \right \}.\label{Eq:Prob_SIC}
%=&\mathrm{Pr}\left \{ h_{j,2}|^2 \geq \! \left [\frac{|h_{j,1}|^2 \mathcal{P} g_{j,1}(\alpha_{j,1})}{\mathcal{P} g_{j,1}(\alpha_{j,1})} \right ] \!\psi \bigg| \left |\varphi \right |\!=\!1, g_{j,1}(\alpha) \right \} \nonumber \\
%=&\mathrm{Pr}\left \{ \frac{h_{j,2}|^2}{h_{j,1}|^2} \geq \! \left [\frac{g_{j,1}(\alpha_{j,1})}{g_{j,1}(\alpha_{j,1})}  \right ] \psi \bigg| \left |\varphi \right |\!=\!1, g_{j,1}(\alpha) \right \} \nonumber \\
%=&\int_{0}^{\frac{g_{j,1}(\alpha_{j,1})}{g_{j,1}(\alpha_{j,1})}} \frac{f_{h2}(h)}{f_{h1}(h)} {dh} \nonumber \\
%=&\int_{0}^{\frac{g_{j,1}(\alpha_{j,1})}{g_{j,1}(\alpha_{j,1})}}  \left (\frac{z_{1}^2}{z_{2}^2} \frac{C_2\sqrt{C_2}}{C_1\sqrt{C_1}} \right ) \frac{I_o\left ( \sqrt{2K_2}\sqrt{C_2} \right )}{I_o\left ( \sqrt{2K_1}\sqrt{C_1} \right )} \nonumber \\ 
%& \centerdot \textrm{exp} \left \{ -\frac{1}{2}\! \left [-\frac{1}{C_1} \!+\! \frac{1}{C_2} \!+\! K_1 \!-\! K_2 \!-\!Y_1^{2} \!-\!Y_2^{2} \right ]  \right \} {dh}
\end{align}

Note that, in (\ref{Eq:Prob_SIC}) we assume\footnote{For the sake of simplicity in mathematical notation, in (\ref{Eq:Prob_SIC}) we also consider $\Theta_{j,2}(\alpha)=\Theta_{j,2}(\alpha_{j,2})$, as well as $g_{j,1}(\alpha)=g_{j,1}(\alpha_{j,1})$.} the cardinality $\left | \varphi   \right |=1$, indicating that only one interfered transmission message was considered. The interfered signal is represented by $P^{2'}_{j,2}$ transmitted in the ascending orbit (which could be a projected power level $\mathcal{L}_2$ with FTP scheme). On the other hand, the reference\footnote{Note that, the interested signal is represented by subscript $1$, while the interference signal is assumed with subscript $2$.} signal is assumed as $P^{1'}_{j,1}$, the message sent by device $u=1$ in the same satellite lap $j$.


\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{figuras/Prob_theta_2024_March.eps}
    \caption{Capture probability $\Theta_{j,u}$ for the first four devices in the $j=1$ satellite lap time, considering the common power level $\mathcal{L}_{1}=-123.64$ dBm and threshold $\psi=1$ dB.} 
    \label{fig:DtS_probSIR}
\end{figure}


\subsection{Energy Consumption}


We have also expanded our analysis to include system energy consumption. Thus, we define the energy efficiency in the satellite lap $EE_{j}$, for $j \in \{1,..., J\}$, as the ratio between the power energy expended with the average number of successful uplinks per total energy consumed during the satellite lap. According to the proposed DtS FTP and CTP, the transmission power of each device should be different since they used fixed or control schemes. Therefore, it can be expressed as:
\begin{equation}
    EE_j=\frac{\sum\limits_{ \forall u \subseteq \mathbb{P}_j}^{}Pt_{j,u}}{\sum\limits_{ u=1}^{U}Pt_{j,u}}, 
    \label{Eq:EE_j}
\end{equation}
where, the numerator of (\ref{Eq:EE_j}) represents the total energy used by the devices contained in set $\mathbb{P}_m$, that successfully decoded their packets at the satellite gateway in that lap.  



\section{Summary of the simulation scenario and Parameters}
\label{Sec:Summary_parameters}

In this section, we resume all details concerning the overall implementation. The next section presents the simulated results considering the following LoRa-based works~\cite{Alonso.23, Alvarez.22, Jean.24} exposed in Table.~\ref{tab:simulation_Parameters}. The IoT network is over the country of France. In a realistic scenario of DtS-IoT, the device locations are uniformly distributed according to geographic coordinates using the Python GeoPy library~\cite{GeoPy}. The distance between each $u$ device and the gateway is estimated with the Skyfield astronomy library~\cite{Skyfield}. Utilizing data sourced from the CelesTrack platform~\cite{Celestrack}, this public library fits information in the two-line element (TLE) set format to determine the satellite's locations based on its orbit and pointing time. More specifically, the satellite visibility times allows to compute the distance in kilometers using~\cite{blufftonSkyfield}. Thus, we applied the proposed non-orthogonal schemes with fixed and controlled transmission power using MatLab\raisebox{1ex}. Furthermore, we take into account the real orbit of the LacunaSat-3 LEO satellite, positioned at an altitude ranging from $500$~km to $600$~km above Earth~\cite{LacunaLaunch.2020}. As indicated by the works~\cite{Alvarez.22,Alonso.23}, we also assume a minimum elevation angle of $30^{\circ}$, to establish  the satellite footprint. 


\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{figuras/Th_uplinks_51bytes.eps} %France_T200_sic.eps
    \caption{The average number of uplinks for a total number of devices $U=200$, applying DtS-IoT schemes FTP (blue line), ALOHA protocol (burnt yellow line), and CTP (black line) for a LoRa payload size of $51$ bytes} 
    \label{fig:Th_DtS_schemes}
\end{figure}

\begin{table}[!t]
\caption{\justifying Direct-LoRa-Satellite uplink simulation parameters.}
\centering
\begin{tabular}{lrc}
\hline
\multicolumn{1}{c}{Parameters} & \multicolumn{1}{c}{LoRa} & \multicolumn{1}{l}{Param.}     \\ \hline
Transmission Power             & $14$ {[}dBm{]}          &      $P_t$                       \\
Transmitter Antenna Gain \hspace{0.5cm}      & 0 {[}dBi{]} &    $G_{t}$                    \\
Receiver Antenna Gain         & $13.5$ {[}dBi{]}           &    $G_{r}$              \\
Channel Bandwidth              & $125$ {[}kHz{]}            &   $B$                           \\
Frequency band of Europe       & $868$ {[}MHz{]}           &      $f_{req}$                        \\
Time-on-Air                    & $27935$ {[}ms{]}           &      $ToA$                        \\
Payload size                   & $51$ {[}Bytes{]}           &      -                        \\
Spread Factor                  & $12$                       &         $SF$                     \\
Sensitivity                    & $-137$ {[}dBm{]}           &         -                \\
SNR Threshold                  & $-20$ {[}dB{]}             &      $\gamma$                 \\
Interference Threshold         & $1$ {[}dB{]}               &     $\psi$                 \\ \hline
\end{tabular}
\label{tab:simulation_Parameters}
\end{table}


\section{Numerical Results}

In this section we present the simulation results to evaluate the trade-off between the average number of successfully decoded transmissions and energy consumption considering the regular ALOHA protocol and the proposed MAC direct-to-satellite schemes FTP and CTP.



\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{figuras/Th_uplinks_20bytes.eps} %France_T200_sic.eps
    \caption{The average number of uplinks for a total number of devices $U=200$, applying DtS-IoT schemes FTP (blue line), ALOHA protocol (burnt yellow line), and CTP (black line) for a LoRa payload size of $20$ bytes.} 
    \label{fig:Th_DtS_schemes_20B}
\end{figure}

Using a threshold value similar to previous LoRa studies~\cite{Jean.20,Alonso.23,Maleki.23}, Fig.~\ref{fig:DtS_SIR} depicts the Signal-to-Interference Ratio (SIR), considering the same four devices mentioned in Section~\ref{Sec:DtS-Schemes}. However, in this case, the interference term in Equation (\ref{Eq:prob_SIR}) incorporates the received power value at the common initial level $\mathcal{L}_1=-123.64$ dBm. Subsequently, Fig.~\ref{fig:DtS_probSIR} presents the outage probability, using the threshold parameter $\psi=1$dB, to ensure the successful decoding of both the received interest packet and the interference message. In our study, we have assumed an outage probability in the presence of interference to be $10\%$ of the ratio between the received and interference signals. In other words, due to the circle markers in color magenta, Fig.~\ref{fig:DtS_probSIR} also show a respective instants and/or elevation angles to operate and decode our messages with interference. Given these received power levels to decode collisions at the satellite, we can determine the desired value of the second level as $\mathcal{L}_2=-120.70$ dBm. 



Fig.\ref{fig:Th_DtS_schemes} shows the average number of successfully decode uplinks considering FTP, ALOHA and CTP strategies considering a payload size of $51$ bytes. Respectively, lines in blue, burnt yellow and black line colors. All tree mechanisms are very similar in the beginning of the network size (lower than $U=30$). However, after a total number of IoT devices $U=50$, the fixed transmission power (FTP) outperforms the others. The burnt yellow line represents the performance of ALOHA protocol, as we know,random IoT transmissions generates a lot of collision messages. To illustrate this issue, Fig.~\ref{fig:Collision} shows an collision histogram for ALOHA (burnt yellow columns), FTP (blue contour columns) and (black contour columns). In vertical graphical axes indicates the quantity of collision messages. In the horizontal axes, Type-0 means that no collisions were detected, while Type-1 show that double collision were detected at same time, and so on. We expected that the CTP method to converge towards ALOHA, as it adjusts the power to ensure that the selected level of received power can reach the satellite. Furthermore, the blue bars highlight that the FTP scheme exhibits the highest number of non-collided packets, comprising nearly $25\%$ ($10\%$ fewer collisions) of the total messages, with an additional $30\%$ experiencing double messages. Notably, when planning IoT power messages, Type-1 collisions are easier to decode using the SIC procedure.



\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{figuras/Histo_collisions_II.eps}
    \caption{Collision histogram for $U=120$ using ALOHA (burnt yellow), FTP (blue) and (black) protocols \textit{versus} the type of collisions (no collisions, simple, double, and so on).} 
    \label{fig:Collision}
\end{figure}


In the same direction like \cite{Alonso.23}, we use Table~\ref{tab:simulation_Parameters} changing the payload size for LoRa/LoRaWAN to $20$ bytes. Fig. \ref{fig:Th_DtS_schemes_20B} demonstrates that not only does the average number of successful uplinks increase as the network size grows, but also the performance difference since we compare ALOHA and CTP techniques with FTP. In the worst-case scenario with $2\times10^{2}$ devices, the blue line highlights that we improve the average number of uplinks by nearly $34\%$ by implementing the non-orthogonal power scheme FTP. Although the CTP protocol can control the transmission power to generate the planned power level at the satellite gateway, two events still affect its throughput performance. Firstly, in CTP, each IoT device utilizes a random process to choose its time to transmit the data packet. Furthermore, based on the projected receive power levels, they also need to decide between $\mathcal{L}_1$ or $\mathcal{L}_2$ levels. Secondly, due to the similar behavior of the number of collided uplinks towards the ALOHA protocol, it's worth noting that two devices may choose to transmit simultaneously and can also choose to generate the same power level. This scenario is detrimental and not sufficiently conducive to decoding both messages using SIC.

\begin{figure}[!t]
    \centering
    \includegraphics[width=\columnwidth]{figuras/EE_uplinks_51bytes.eps}%Energy_Efficiency_March.eps
    \caption{Energy efficiency for total number of device $U=200$ applying FTP (blue line), ALOHA protocol (burnt yellow line), CTP (black line) for a LoRa payload size of $51$ bytes.} 
    \label{fig:Energy_Effic_DtS_schemes_51B}
\end{figure}



\begin{figure}[!ht]
    \centering
    \includegraphics[width=\columnwidth]{figuras/EE_uplinks_20bytes.eps}%Energy_Efficiency_March.eps
    \caption{Energy efficiency for total number of device $U=200$ applying FTP (blue line), ALOHA protocol (burnt yellow line), CTP (black line) for a LoRa payload size of $20$ bytes.} 
    \label{fig:Energy_Effic_DtS_schemes_20B}
\end{figure}

The energy efficiency performance is illustrated in Fig.~\ref{fig:Energy_Effic_DtS_schemes_51B}. For a payload of $51$ bytes, FTP outperform the ALOHA and CTP protocols. The FTP and ALOHA approaches utilize a fixed power value of $14$ dBm for the uplink transmissions, which implies a direct trade-off between the average number of successful messages and power consumption. Comparing the proposed schemes, FTP improve the energy efficiency with difference by more than $10\%$ for a total of $60$ IoT devices. In contrast, the CTP scheme offers the flexibility to optimize system power requirements, likely by dynamically adjusting transmission power based on various factors. However, Fig~\ref{fig:Energy_Effic_DtS_schemes_20B} shows that the energy efficiency performance of the CTP is closer than FTP. It is a consequence of the increasing of average number of successfully uplinks when we decreasing the payload size to $20$ bytes. Indeed, FTP outperforms ALOHA due to its reduced collision rate and higher occurrence of simple collisions, which could be efficiently resolved at the receiver's side.









\section{Conclusion}


This work presents two novel uplink transmission techniques for DtS-IoT. We plan that IoT devices can generate predetermined power levels received at the satellite gateway. Specifically, we evaluate the number of successfully decoded messages and the power consumption considering both schemes, FTP and CTP. We recognize that the potential of the CTP scheme needs to be explored in terms of throughput. In future work, our IoT devices could be embedded with intelligence to optimize the signal level received at the LEO gateway. %We believe that incorporating learning feedback can further improve the numerical results presented in this study. 

\iffalse
\appendices
\section{Proof of definition 1}
Based on the connection probability in~(\ref{Eq:Connec_prob}), we have:
\begin{align*}
 \Phi_{j,u}(\alpha)&= \int_{0}^{\infty}  \frac{z}{\sigma^{2}\mathcal{S}^{2}} \times \frac{1}{\beta \sigma \mathcal{S} \sqrt{2\pi}}   \\
& \times \mathrm{exp}\left [ -\frac{1}{2} \left ( \frac{\textrm{ln} \ S - \mu}{\beta \sigma} \right )^{2} -\frac{1}{2} \left ( \frac{z^{2}}{\sigma^{2} \mathcal{S}^{2}}+2K \right ) \right ] \\ 
&\times I_o\left( \frac{z}{\sigma \mathcal{S}}\sqrt{2K} \right) \\
&=\frac{1}{\beta \sqrt{2\pi}} \int_{0}^{\infty} \frac{z^2}{z \sigma^{2}\mathcal{S}^{2}} \times \textrm{exp} \left [ -\frac{1}{2} \left ( C +2K + y^{2} \right ) \right ] \\ 
&\times I_o\left( \frac{z}{\sigma \mathcal{S}}\sqrt{2K} \right) \\
&=\frac{1}{\beta \sqrt{2\pi}} \int_{0}^{\infty} \frac{C}{z} \times \textrm{exp} \left [ -\frac{1}{2} \left ( C +2K + y^{2} \right ) \right ] \\
&\times I_o\left( \sqrt{C}\sqrt{2K} \right) 
\end{align*}
\fi
% you can choose not to have a title for an appendix
% if you want by leaving the argument blank


\bibliographystyle{IEEEtran}
\bibliography{IEEEabrv,references}

\end{document}



